Map-Assisted Remote-Sensing Image Compression at Extremely Low Bitrates

Remote-sensing (RS) image compression at extremely low bitrates has always been a challenging task in practical scenarios like edge device storage and narrow bandwidth transmission. Generative models including VAEs and GANs have been explored to compress RS images into extremely low-bitrate streams. However, these generative models struggle to reconstruct visually plausible images due to the highly ill-posed nature of extremely low-bitrate image compression. To this end, we propose an image compression framework that utilizes a pre-trained diffusion model with powerful natural image priors to achieve high-realism reconstructions. However, diffusion models tend to hallucinate small structures and textures due to the significant information loss at limited bitrates. Thus, we introduce vector maps as semantic and structural guidance and propose a novel image compression approach named Map-Assisted Generative Compression (MAGC). MAGC employs a two-stage pipeline to compress and decompress RS images at extremely low bitrates. The first stage maps an image into a latent representation, which is then further compressed in a VAE architecture to save bitrates and serves as implicit guidance in the subsequent diffusion process. The second stage conducts a conditional diffusion model to generate a visually pleasing and semantically accurate result using implicit guidance and explicit semantic guidance. Quantitative and qualitative comparisons show that our method outperforms standard codecs and other learning-based methods in terms of perceptual quality and semantic accuracy. The dataset and code will be publicly available at https://github.com/WHUyyx/MAGC.

==> sec/0_abstract.tex <==
\begin{abstract}
Remote-sensing (RS) image compression at extremely low bitrates has always been a challenging task in practical scenarios like edge device storage and narrow bandwidth transmission. Generative models including VAEs and GANs have been explored to compress RS images into extremely low-bitrate streams. However, these generative models struggle to reconstruct visually plausible images due to the highly ill-posed nature of extremely low-bitrate image compression. To this end, we propose an image compression framework that utilizes a pre-trained diffusion model with powerful natural image priors to achieve high-realism reconstructions. However, diffusion models tend to hallucinate small structures and textures due to the significant information loss at limited bitrates. Thus, we introduce vector maps as semantic and structural guidance and propose a novel image compression approach named Map-Assisted Generative Compression (MAGC). MAGC employs a two-stage pipeline to compress and decompress RS images at extremely low bitrates. The first stage maps an image into a latent representation, which is then further compressed in a VAE architecture to save bitrates and serves as implicit guidance in the subsequent diffusion process. The second stage conducts a conditional diffusion model to generate a visually pleasing and semantically accurate result using implicit guidance and explicit semantic guidance. Quantitative and qualitative comparisons show that our method outperforms standard codecs and other learning-based methods in terms of perceptual quality and semantic accuracy. The dataset and code will be publicly available at https://github.com/WHUyyx/MAGC.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
Satellites capture large volumes of high-resolution images of the Earth’s surface, resulting in an exponential growth of newly captured remote-sensing (RS) images every day. There exists a demand for extremely low-bitrate RS image compression techniques in practical scenarios, such as efficient long-term storage and analysis in cloud-based systems with storage limitations, and faster data transfer in emergency communication networks that may be constrained. The main challenge is to develop effective compression techniques that substantially reduce the bitrate while preserving essential RS image features, enabling accurate and reliable use of compressed images in various remote sensing applications \citep{tgrs2024}.
% High-throughput onboard hyperspectral image compression with ground-based CNN reconstruction
% Remote Sensing Image Compression Based on High-Frequency and Low-Frequency Components

In the past decades, the majority of image compression methods were designed upon frequency analysis, such as JPEG \citep{jpeg}, JPEG2000 \citep{jpeg2000}, BPG \citep{bpg} and VTM \citep{vtm}. These approaches generally employ a block-based transform coding framework and rely on hand-crafted features and heuristics to reduce redundancy in original images. At extremely low bitrates, traditional compression techniques can lead to significant loss of information. This loss can compromise the utility of the RS images for interpretation and analysis, as crucial features such as terrain, vegetation, and urban structures might be blurred or completely lost.
% The jpeg still picture compression standard
% Jpeg2000: Image compression fundamentals, standards and practice
% Bpg image format
% Versatile video coding
% Dynamic Kernel-Based Adaptive Spatial Aggregation for Learned Image Compression



Recently, learned image compression methods have shown remarkable performance compared to traditional codecs \citep{channelwise, checkerboard, stf, elic, mixed}. Ballé et al. \citep{hyperprior} first proposed a learned image compression framework based on a variational autoencoder (VAE) architecture, as shown in Fig.\:\hyperref[fig1]{1(a)}. The encoder performs downsampling on the input image, yielding a compact latent representation that contains the most information about the original image. After quantization, the latent is transformed to a bitstream via entropy coding. On the decoding side, the image is reconstructed through the decoder. The entropy model is designed for distribution parameter estimation and probabilistic prediction for entropy coding to further reduce the bitrates. The learned image compression framework employs a data-driven, end-to-end training strategy, adaptively learning weights based on image contents. Consequently, the end-to-end learning approach outperforms traditional coding schemes where performance is limited by the handcrafted and fixed coding frameworks. However, these MSE-optimized VAE-based models tend to produce blurred results at low bitrates, limiting their practicality in such extreme low-bitrate scenarios.
% CHANNEL-WISE AUTOREGRESSIVE ENTROPY MODELS FOR LEARNED IMAGE COMPRESSION
% Checkerboard Context Model for Efficient Learned Image Compression
% The devil is in the details Window-based attention for image compression
% Efficient learned image compression with unevenly grouped space-channel contextual adaptive coding
% Learned Image Compression with Mixed Transformer-CNN Architectures
% VARIATIONAL IMAGE COMPRESSION WITH A SCALE HYPERPRIOR
% Neural datadependent transform for learned image compression


Considering the requirement of improving the perceptual quality of reconstructed images, researchers have proposed generative image compression frameworks based on generative adversarial network (GAN) \citep{gan} and diffusion model \citep{ddpm}, as shown in Fig.\:\hyperref[fig1]{1(b)} and Fig.\:\hyperref[fig1]{1(c)}. GAN-based methods additionally use a discriminator to distinguish real images from the images generated by the decoder \citep{1804, compressnet, hific, multirealism, illm}. Diffusion-based methods usually regard the quantized latent as a condition used for a denoising diffusion process \citep{cdc, diffusion}. Unlike VAE-based methods that focus on the rate-distortion trade-off, these methods typically adopt a rate-distortion-perception trade-off during the training process \citep{rethinking}, dramatically improving the visual quality of reconstructed images.
% Generative Adversarial Networks for Extreme Learned Image Compression
% CompressNet Generative Compression at Extremely Low Bitrates
% High-Fidelity Generative Image Compression
% Multi-Realism Image Compression with a Conditional Generator
% Improving Statistical Fidelity for Neural Image Compression with Implicit Local Likelihood Models
% Lossy Image Compression with Conditional Diffusion Models
% DiffusionAutoencoders:TowardaMeaningfulandDecodableRepresentation
% Rethinking Lossy Compression The Rate-Distortion-Perception Tradeoff



 
\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{fig_pdf/fig1.pdf}
\captionsetup{singlelinecheck=false} % 左对齐
\caption{Operational diagrams of learned image comprssion frameworks. Q denotes quantization. EM represents the entropy model. D denotes the discriminator. \begin{math}\mathcal{E}\end{math} and $\mathcal{D}$ denote the pre-trained SD VAE encoder and decoder used to transform data between pixel space and latent space.}
\label{fig1} 
\end{figure*} 


The compression approaches mentioned above exhibit acceptable performance only at normal bitrates. However, at extremely low bitrates, i.e., less than 0.1 bits per pixel (bpp), VAE-based methods tend to produce severe blurriness \citep{1804}, while GAN-based methods can introduce erroneous textures \citep{sketch}. Recently, the Stable Diffusion (SD) model has been utilized as a generative prior in extremely low-bitrate image compression \citep{sketch, 2211, iclr2024}. With the powerful image priors and the generative capability of the pre-trained model, SD-based methods have demonstrated the characteristics of being less reliant on bitrates \citep{iclr2024}. However, these methods achieve extremely low bitrates by using text descriptions or sketches extracted from images to be compressed, significantly removing most of the information from the original images. Thus, the compressed bitstream cannot provide sufficient conditions for image generation and results in noticeable compression distortion. To extract essential information as effective conditions for the denoising diffusion process, we propose a novel SD-based image compression framework as shown in Fig.\:\hyperref[fig1]{1(d)}. We employ $\text{g}_\text{a}(\cdot)$ and $\text{g}_\text{s}(\cdot)$ to further compress and decompress the latent representation $z_0$, and the reverse diffusion process is conditioned on compressed latent representation $\hat{z}$ as implicit guidance to create realistic RS images.
% Text + Sketch Image Compression at Ultra Low Rates
% EXTREME GENERATIVE IMAGE COMPRESSION BY LEARNING TEXT EMBEDDING FROM DIFFUSION MODELS
% TOWARDS IMAGE COMPRESSION WITH PERFECT REALISM AT ULTRA-LOW BITRATES

Existing SD-based methods typically take full advantage of explicit conditions, such as text and sketches, which are not suitable for RS images characterized by complex and irregular ground objects. This is because the network cannot extract accurate semantic information from these conditions. For instance, when given a textual prompt like ``many houses are on both sides of the road'', the diffusion model fails to understand the precise locations of the road and houses, leading to semantically incorrect reconstructions. Therefore, to minimize semantic distortion in compressed RS images at low bitrates, it is imperative to employ explicit guidance that encapsulates spatially accurate semantic information of the original RS images.

A vector map is a graphical representation of geospatial data in which map elements such as roads and buildings are represented by geometric shapes and coordinates such as spatially positioned lines and polygons. This type of data provides semantic and structural information of ground objects and can be leveraged as semantic guidance during RS image compression and decompression. In many real-world applications, vector maps are already available or required for other purposes, such as navigation, urban planning, or geographic information systems. Utilizing these existing resources for image compression does not impose significant additional storage burdens. 
%If not, we can also store only one copy of the vector map, which requires significantly less storage space compared to rasterized RS images, on both the compression and decompression sides, and efficiently reuse it for RS images captured periodically from different satellites. 
Inspired by this, we propose an extremely low-bitrate image compression approach for RS images, named Map-Assisted Generative Compression (MAGC), which utilizes semantic information from vector maps with the pre-trained SD model to reconstruct RS images at extremely low bitrates. Specifically, we conduct the denoising diffusion process using the compressed latent representations as implicit guidance and vector maps as explicit guidance. Under implicit and explicit guidance, our MAGC can generate images with higher fidelity and better maintain semantic integrity compared to other methods. We conduct the semantic segmentation task and the experimental results indicate that our method can save 90\% bitrates than VTM-23.3 \citep{vtm} and 60\% bitrates than MS-ILLM \citep{illm} with even higher mIoU.
% Semantic Guided Large Scale Factor Remote Sensing Image Super resolution with Generative Diffusion Prior


Main contributions of this paper are as follows: 
\begin{enumerate}[1)]
\item We propose the Map-Assisted Generative Compression (MAGC) model, which integrates semantic information from vector maps into a pre-trained SD model to generate images with plausible visual quality and accurate semantic features.
\item We develop a VAE-based latent compression module (LCM) to further compress the latent representations and provide implicit guidance for the denoising diffusion process. The semantic adapter module (SAM) is employed to extract multi-scale features from vector maps as explicit guidance to generate semantically accurate images.
\item Experimental results indicate that our method outperforms others in perceptual quality and semantic accuracy. Semantic segmentation results show that our method can save 90\% bitrates than VTM-23.3 and 60\% bitrates than MS-ILLM with even better performance.  
\end{enumerate}

The rest of this paper is organized as follows. Section \ref{section2} gives a review of image compression techniques. The framework of MAGC is illustrated in Section \ref{section3}. Section \ref{section4} compares the performance of the proposed MAGC with different compression methods. In Section \ref{section5}, we conduct ablation studies and discuss the impact of each component. Finally, we summarize this paper in Section \ref{section6}.

==> sec/2_related_work.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Related Work (引用数：24)
\section{Related Work}\label{section2}
In this section, we present a review of image compression from the following three subfields: learned image compression models, image compression at extremely low bitrates and RS image compression.

\subsection{Learned Image Compression Models}
Over the last few years, learned image compression has made great progress and demonstrated outstanding performance. The pioneering work of Ballé et al. \citep{end-to-end} first proposed a CNN-based end-to-end learned image compression framework that uses stacked convolution layers and generalized divisive normalization (GDN) layers to achieve transform coding. Then they modified the framework as a VAE-based model and introduced a hyperprior as side information \citep{hyperprior}. Furthermore, some researchers proposed to integrate a context model with hyperprior to achieve more accurate probabilistic predictions of the latent representation \citep{channelwise,checkerboard, elic, joint}. In addition to the refinement of entropy models, multiple novel and efficient CNN-based transforms have been proposed \citep{ elic,cheng2020, tang}. Besides, inspired by the success of Vision Transformer in many vision tasks \citep{vit}, Swin-Transformer-based methods have been explored in learned image compression \citep{ stf, transformer-based}. Liu et al. \citep{mixed} proposed an efficient parallel Transformer-CNN Mixture block to improve the overall architecture of image compression models by incorporating the local modeling ability of CNN and the non-local modeling ability of transformer.
% END-TO-END OPTIMIZED IMAGE COMPRESSION
% Joint Autoregressive and Hierarchical Priors for Learned Image Compression
% Learned Image Compression with Discretized Gaussian Mixture Likelihoods and Attention Modules
% tang:Joint graph attention and asymmetric convolutional neural network for deep image compression
% vit: 
% Transformer-based transform coding



Additionally researchers have explored GAN-based and diffusion-based methods to enhance the visual quality of the reconstructed images. Based on theoretical research of the rate-perception-distortion trade-off \citep{rethinking}, many conditional GAN-based approaches \citep{hific, multirealism, illm} have been proposed. Mentzer et al. \citep{hific} proposed a novel generative image compression framework using a conditional GAN architecture. Agustsson et al. \citep{multirealism} proposed an improved decoder that navigates the distortion-realism trade-off. Muckley et al. \citep{illm} introduced an improved non-binary discriminator that is conditioned on quantized local image representations and achieve state-of-the-art perceptual quality. In contrast to these GAN-based methods, some diffusion-based methods \citep{cdc, diffusion} also show comparable performance at normal bitrates using conditional Gaussian diffusion \citep{ddpm}, but they show less stability at extremely low bitrates.
% Hoogeboom: High-fidelity image compression with score-based generative models.
% Denoising Diffusion Probabilistic Models


\subsection{Image Compression at Extremely Low Bitrates}
% Besides, Invertible Neural Network (INN) \citep{inn} and text-guided \citep{2304} methods have also been adopted in extremely low-bit compression. 
Under the extreme low-bitrate conditions, GAN-based compression methods \citep{1804, compressnet,hific,  1703, iwai, cvpr2024} have demonstrated superior performance compared to MSE-optimized VAE-based models and standard codecs. For instance, Sauturkar et al. \citep{1703} proposed a pioneering approach of generative compression utilizing a generative adversarial strategy and demonstrated impressive results. Mentzer et al. \citep{hific} incorporated rate-distortion-perceptual trade-off with a GAN-based framework, yielding reconstructions with high realism, even at 0.1bpp on the CLIC2020 test set and 0.2bpp on Kodak dataset. Jia et al. \citep{cvpr2024} introduced a Generative Latent Coding architecture that maintains high visual quality with less than 0.04 bpp on natural images and less than 0.01 bpp on facial images. Besides, text-guided transforms have also been adopted in extremely low-bitrate image compression \citep{2304}.
% Generative Compression
% Fidelity-Controllable Extreme Image Compression with Generative Adversarial Networks
% Generative Latent Coding for Ultra-Low Bitrate Image Compression
% Extremely Low Bit-rate Image Compression via Invertible Image Generation
% Multi-Modality Deep Network for Extreme Learned Image Compression



% cheng+sd,  text+sketch, iclr2024
With powerful image priors and generative capability, the pre-trained text-to-image model, such as the SD model, has been used in extremely low-bitrate image compression. For instance, Pan et al. \citep{2211} adopted learnable text embeddings and pre-trained diffusion model to generate realistic images. Lei et al. \citep{sketch} extracted textual descriptions and sketches from the original images to guide image generation. Furthermore, Careil et al. \citep{iclr2024} conditioned the diffusion model on more versatile end-to-end learned vector-quantized image features, maintaining the ability to reconstruct realistic images at ultra-low bitrate (e.g., less than 0.01 bpp). 


\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{fig_pdf/fig2.pdf}
\captionsetup{singlelinecheck=false} % 左对齐
\caption{The two-stage pipeline of the proposed MAGC. In the first stage, the latent compression module (LCM) is designed to compress the latent representation and provide implicit guidance for the conditional diffusion model. In the second stage, the semantic adapter module (SAM) is utilized to produce multi-scale features, serving as explicit guidance for the conditional diffusion process.}
\label{fig2}
\end{figure*} 

\subsection{RS Image Compression}
In the last few decades, there has been a surge in the volume of RS images, necessitating the development of effective image compression techniques. In early stages, some standard codecs based on traditional transform coding, such as JPEG and JPEG2000, were extensively applied to RS image compression \citep{JPEG2000-1, JPEG2000-2, JPEG2000-3}. These methods performed transforms from the image domain to the frequency domain, followed by quantization, and achieved significant bitrate savings. Additionally, based on the discrete wavelet transform, the Consultative Committee for Space Data Systems (CCSDS) has also been utilized before the popularity of learning-based approaches \citep{CCSDS-1, CCSDS-2}. However, prior work \citep{Efficient} has shown that severe blurriness and artifacts are prevalent in handcrafted transform coding methods, especially at low bitrates. To address this issue, some learned image compression methods have been explored for RS image compression.
% 3：JPEG2000 coding strategies for hyperspectral data. A cartoon-texture approach for JPEG/JPEG 2000 decompression based on TGV and shearlet transform. JPEG2000 encoding of remote sensing multispectral images with no-data regions
% 4: Extending the CCSDS recommendation for image data compression for remote sensing scenarios. A 13.3 Gbps 9/7M discrete wavelet transform for CCSDS 122.0-B-1 image data compression on a spacegrade SRAM FPGA,
% 5:Efficient and effective context-based convolutional entropy modeling for image compression


Encouraged by the success of VAE-based methods in natural image compression, some researchers have proposed using these models to compress RS images \citep{ tgrs2024,uplink, Oliveira, fu, Chong, xiang-long-range}. Chong et al. \citep{Chong} incorporated the Markov Random Field into the attention mechanism and showed impressive results on standard RS datasets of varying resolutions. Wang et al. \citep{uplink} used historical images as reference images for on-orbit compression based on uplink transmission procedures. Considering the reconstruction of high-frequency features such as edge information and texture characteristics, Xiang et al. \citep{tgrs2024} incorporated a dual-branch architecture based on high-frequency and low-frequency feature components. 

% Oliveira: Satellite image compression and denoising with neural networks
% Fu: Remote Sensing Image Compression Based on the Multiple Prior Information
% Chong: High-Order Markov Random Field as Attention Network for High-Resolution Remote-Sensing Image Compression
% XIANG: Remote sensing image compression with long-range convolution and improved non-local attention model

In addition to the VAE-based methods, GAN-based methods have also been developed to generate realistic RS images. Zhao et al. \citep{zhao-symmetrical} adopted several pairs of symmetrical encoder-decoder lattices and multiple discriminators to enhance edges, contours and textures in the reconstructed images. Han et al. \citep{edge} proposed an edge-guided adversarial network to simultaneously restore edge structures and generate texture details. Pan et al. \citep{tgrs2023} presented a coupled compression generation network that reconstructs image content and detailed textures separately and achieves outstanding results in the DOTA dataset at extremely low bitrates.
% Zhao: Symmetrical lattice generative adversarial network for remote sensing images compression
% Han: Edge-Guided Remote-Sensing Image Compression
% A Coupled Compression Generation Network for Remote-Sensing Images at Extremely Low Bitrates

These learning-based approaches mentioned above have shown outstanding performance in RS image compression. However, they generally focused on improving pixel-level fidelity or perceptual quality of the reconstructed images, while neglecting semantic integrity which is of paramount significance for RS images. To this end, introducing vector maps as semantic guidance in RS image compression is a promising strategy that maintains a higher degree of semantic integrity even at extremely low bitrates.
% 引用数：24

==> sec/3_method.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Proposed Method
\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{fig_pdf/fig3.pdf}
\captionsetup{singlelinecheck=false} % 左对齐
\caption{The network architecture of the proposed LCM, consists of the latent transform networks, hyperprior networks and a channel-wise context model. \textit{Q} represents quantization. \textit{AE}, \textit{AD} represent arithmetic encoder and arithmetic decoder. $\downarrow$ and $\uparrow$ indicate downsampling and upsampling. We set \textit{N} = 128 and \textit{M} = 64 in our experiments.}
\label{fig3}
\end{figure*} 

\section{Proposed Method}\label{section3}
\subsection{Overview}
In this section, we give an overview of the proposed MAGC. As shown in Fig.\:\hyperref[fig2]{2}, our MAGC consists of two stages. In the first stage, the image is mapped into a latent representation via a pre-trained SD VAE encoder. Then the latent representation is compressed, quantized, transmitted and decompressed in the LCM. The compressed latent representation, containing the majority of the information from the original image, provides implicit guidance for the conditional diffusion model and ensures that the reconstructed image contains the same contents as the original one. The process of the first stage can be formulated as follows:
\begin{align}
    z_0&=\mathcal{E}(x), \\
    \hat{z}&=\text{LCM} (z_0, m) 
\end{align}
where $\mathcal{E}(\cdot)$ denotes the pre-trained SD VAE encoder. $x$ denotes the input image. $z_0$ and $\hat{z}$ are the original and compressed latent representation. $m$ represents the vector map.

In the second stage, we utilize the SAM to produce multi-scale features as explicit guidance, which provides additional semantic and structural information and assists in generating images with semantic accuracy. Under implicit guidance from the compressed latent representation and explicit guidance from the vector map, the conditional diffusion model is conducted in the latent space, followed by the generation of the realistic and semantically accurate reconstruction through a pre-trained SD VAE decoder. The process can be formulated as follows:
\begin{align}
f_{\text{ms}}&=\text{SAM}(\text{SE}(m), z_t), \\
\tilde{z}_0&=\text{CDM}(\hat{z},f_{\text{ms}}), \\
\hat{x}&=\mathcal{D}(\tilde{z}_0),
\end{align}
where 
$\text{SE}$ denotes the semantic encoder. 
$f_{\text{ms}}$ is the produced multi-scale features. 
$z_t$ and $\tilde{z}_0$ are the noised and denoised latent representation. $\text{CDM}$ denotes the conditional diffusion model. $\mathcal{D}(\cdot)$ denotes the pre-trained SD VAE decoder. $\hat{x}$ is the reconstructed image.

\subsection{Latent Compression Module}
The LCM is designed to further reduce the redundancy of the latent representation and provide implicit guidance for the denoising diffusion process. The network architecture of LCM is illustrated in Fig.\:\hyperref[fig3]{3}. Similar to the VAE-based learned image compression frameworks, the LCM consists of latent transform networks, hyperprior networks and a channel-wise context model. Furthermore, the spatially-adaptive denormalization (SPADE) ResBlock \citep{spade} is designed to integrate the semantic information from vector maps into the latent transform coding. The details of the LCM are presented below.

\subsubsection{VAE-based Latent Coding}
Since Ballé et al. \citep{hyperprior, end-to-end} proposed the VAE-based image compression framework, most of the learned image compression methods have followed the paradigm. Inspired by this, we model the latent compression process using VAE-based networks. The generalized latent compression framework is formulated as follows:
\begin{equation}
\begin{aligned}
    y&=\text{g}_\text{a}(z,m;\phi),   \\
    \hat{y}&=\text{Q}(y),  \\
    \hat{z}&=\text{g}_\text{s}(\hat{y},m;\theta),
\end{aligned}
\end{equation}
where $y$ denotes the compact representation obtained from $z$. $\hat{y}$ denotes the quantized counterpart of $y$. $\text{g}_\text{a}(\cdot)$ and $\text{g}_\text{s}(\cdot)$ are analysis and synthesis transforms. $\phi$ and $\theta$ are learnable parameters of the transform networks. 
$\text{Q}$ represents the quantization operation.

As shown in Fig.\:\hyperref[fig3]{3}, $\text{g}_\text{a}(\cdot)$ consists of several residual blocks and downsampling convolution layers, performing the transform from the input $z$ to the compact representation $y$ in the encoding process. Symmetrical to this, $\text{g}_\text{s}(\cdot)$ employs the pixelshuffle operation to perform upsampling and maps $\hat{y}$ back to $\hat{z}$. In contrast to previous methods that inject uniform noise during training to simulate the quantization error, we employ the straight-through estimator (STE) \citep{illm, ste} to pass the quantized to the decoder with backpropagation, ensuring that the decoder sees the same data distribution during training and inference.
%ste: Lossy image compression with compressive autoencoders 

Following the previous work \citep{joint}, We model each element of $\hat{y}$ as a single Gaussian distribution, and the standard deviations $\sigma$ and means $\mu$ are estimated by the entropy model. To achieve a more precise distribution estimation, the hyperprior networks \citep{hyperprior} and the channel-wise autoregressive context model \citep{channelwise} are introduced in our entropy model. As shown in the right part of Fig.\:\hyperref[fig3]{3}, the hyper encoder $\text{h}_\text{a}(\cdot)$ encodes $y$ into the side information $h$. Then $\hat{y}$ is divided into $K$ slices ($y^1,y^2,...,y^K$) alone the channel dimension, and these slices are encoded and decoded in an autoregressive manner. Specifically, estimating the distribution of the current slice $y^i$ is conditioned on both the hyperprior and the previously decoded symbols $y^{<i}$. The entire entropy model is formulated as follows:
\begin{equation}
\begin{aligned}
    h&=\text{h}_\text{a}(y;\phi_\text{h}),   \\
    \hat{h}&=\text{Q}(h),  \\
    gc&=\text{h}_\text{s}(\hat{h};\theta_\text{h}), \\
    \mu^i, \sigma^i&=\text{g}_\text{cm}(gc,y^{<i};\theta_\text{cm}), 1\leq i\leq K, \\
    p_{\hat{y}}(\hat{y}^i\vert ctx)&=[\mathcal{N}(\mu^i,(\sigma^i)^2)*\text{U}(-\frac{1}{2},\frac{1}{2})](\hat{y}^i) \\
    \text{with}\quad ctx &=(\hat{h},y^{<i},\theta_\text{h},\theta_\text{cm}),
\end{aligned}
\end{equation}
where $\text{h}_\text{a}(\cdot)$, $\text{h}_\text{s}(\cdot)$, $\phi_\text{h}$ and $\theta_\text{h}$ are hyper analysis and synthesis transform and their learnable parameters. $h$ and $\hat{h}$ are the side information and its quantized counterpart. $gc$ represents the global context, which is the output of $\text{h}_\text{s}(\cdot)$. $\text{g}_\text{cm}(\cdot)$ and $\theta_{\text{cm}}$ are the channel-wise context model and its learnable parameters.




\subsubsection{Semantic-Guided Transform}
As shown in Fig.\:\hyperref[fig3]{3}, we utilize the SPADE ResBlock to integrate the semantic information into the latent transform coding at each scale. The structures of the SPADE ResBlock, SPADE block and basic block are illustrated in Fig.\:\hyperref[fig4]{4}. In the SPADE block, we merge the semantic feature map and latent feature map by concatenation as the input of the first basic block. Then the merged feature map is convolved to produce the scale factor $\gamma$ and bias term $\beta$, which are multiplied and added to the normalized input element-wise. The whole process can be formulated as follows:
\begin{equation}
\begin{aligned}
    f_{\text{bn}}&=\text{BatchNorm}(f_{\text{in}}),  \\
    \gamma&=\text{Conv}_\gamma(\text{BasicBlk}([f_{\text{bn}},f_{\text{sem}}])),   \\
    \beta&=\text{Conv}_\beta(\text{BasicBlk}([f_{\text{bn}},f_{\text{sem}}])),  \\
    f_{\text{out}}&=\gamma \otimes f_{\text{bn}} + \beta,  \\
\end{aligned}
\end{equation}
where $f_{\text{in}}$, $f_{\text{bn}}$, $f_{\text{sem}}$ and $f_{\text{out}}$ are the input feature map, normalized feature map, semantic feature map and output of SPADE block. 
$\text{BasicBlk}$ denotes the basic block.
$\gamma$ and $\beta$ are the produced scale factor and bias.
$\text{Conv}_\gamma$ and $\text{Conv}_\beta$ are the convolution layers used to predict $\gamma$ and $\beta$. 
$\otimes$ represents Hadamard product.
With the help of the SPADE block, the global structural information is incorporated into the latent transform coding. In that case, the compressed latent representation is considered to be allocated a lower bitrate for storing coarse content while retaining the essential global structure. 

\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig_pdf/fig4.pdf}
\captionsetup{singlelinecheck=false} % 左对齐
\caption{Structures of ResBlock, SPADE ResBlock, SPADE block and basic block in our work.}
\label{fig4}
\end{figure}

\subsection{Conditional Diffusion Model}
As shown in Fig.\:\hyperref[fig2]{2}, we utilize the pre-trained SD model to generate images with multiple guidance. In this section, we will introduce how SD works and how to use multiple guidance to generate realistic and semantically accurate reconstructions at extremely low bitrates.

\subsubsection{Stable Diffusion}
The classical Denoising Diffusion Probabilistic Model (DDPM) performs adding and removing noise in pixel space \citep{ddpm}, which is time-consuming for both training and inference. In contrast, the SD model conducts the diffusion process in the latent space with a much smaller spatial resolution \citep{ldm}. Generally, it consists of a pre-trained VAE and a corresponding U-Net denoiser. Firstly, the VAE is trained to convert images into latent space and then reconstruct them, which is formulated as follows:
% High-Resolution Image Synthesis with Latent Diffusion Models

\begin{equation}
\begin{aligned}
    z_0&=\mathcal{E}(x),  \\
    \hat{x}&=\mathcal{D}(z_0),   \\
\end{aligned}
\end{equation}
where $x$ and $\hat{x}$ are the input and reconstructed image. 
$z_0$ denotes the latent representation. 
For the latent forward diffusion process, $z_0$ is progressively corrupted by adding Gaussian noise through a Markov chain, which can be described as:
\begin{equation}
\begin{aligned}
    z_t&=\sqrt{\bar{\alpha}_t}z_0+\sqrt{1-\bar{\alpha}_t}\epsilon, \quad \epsilon \sim \mathcal{N}(0, \textbf{I}),
\end{aligned}
\end{equation}
where $z_t$ is the noised latent representation at step $t$. 
$\bar{\alpha}_t$ is a pre-set hyperparameter controlling the intensity of the added noise. 
Then a denoiser function, $\epsilon_\theta$, is trained to estimate the noise injected to $z_t$. The optimization process can be formulated as follows:
\begin{equation}
\begin{aligned}
    \mathcal{L}=\mathbb{E}_{z_0,\epsilon,t}\left\|\epsilon- \epsilon_\theta(z_t,t)  \right\|^2,
\end{aligned}
\end{equation}
where $t$ is the timestep sampled from [0, $T$].
During inference, the input noised latent $z_T$ is randomly sampled from a standard Gaussian distribution. After $T$ iterations of the backward diffusion processes, the denoised latent is mapped back to pixel space by the pre-trained SD VAE decoder $\mathcal{D}(\cdot)$.

\subsubsection{Denoising with Multiple Guidance}
In our work, the denoising diffusion process is conditioned on both implicit and explicit guidance. Specifically, $\hat{z}$, the output of LCM, contains most of the details from the original images, serving as the implicit guidance, while the vector maps provide additional semantic and structural information as explicit guidance. 

For implicit guidance, we concatenate $\hat{z}$ with $z_t$ as the input of the denoising U-Net at each time step. To adapt the modified dimension, we extend the first convolutional layer by increasing the number of channels that corresponds to the channel dimension of $\hat{z}$, i.e. from 4 to 8. The additional channels are initialized to zero during training. Since $\hat{z}$ contains the compressed information from $z_0$, the final output of the denoising process is controlled toward the original latent representation with implicit guidance.

For explicit guidance, we use a semantic encoder to transform the vector map into a semantic feature map, which is then transformed into multi-scale conditional features $f_{\text{ms}}$ in SAM. The network architectures of the semantic encoder and SAM are shown in Fig.\:\hyperref[fig5]{5}. Similar to previous work \citep{adapter}, the vector map is first downsampled to match the dimension of the noised latent $z_t$, and then concatenated with $z_t$ as input to the first residual block, yielding the feature $f_{\text{ms}}^1$. In each subsequent scale, a convolutional layer and two residual blocks are employed to extract corresponding feature $f_{\text{ms}}^i$. Note that the produced multi-scale features $f_{\text{ms}}=\{f_{\text{ms}}^1,f_{\text{ms}}^2,f_{\text{ms}}^3,f_{\text{ms}}^4\}$ have the same dimension with the intermediate features $f_{\text{enc}}=\{f_{\text{enc}}^1,f_{\text{enc}}^2,f_{\text{enc}}^3,f_{\text{enc}}^4\}$ in the encoder side of the U-Net denoiser. These conditional features $f_{\text{ms}}$ are then added with $f_{\text{enc}}$ at each scale. By integrating the explicit guidance with the denoising diffusion process, the reconstructions are considered to be semantically consistent with the original images even at extremely low bitrates.

\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{fig_pdf/fig5.pdf}
\captionsetup{singlelinecheck=false} % 左对齐
\caption{Network architecture of semantic encoder and semantic adapter module (SAM).}
\label{fig5}
\end{figure} 
% T2I-Adapter: Learning Adapters to Dig out More Controllable Ability for Text-to-Image Diffusion Models
% DiffBIR Towards Blind Image Restoration with Generative Diffusion Prior

\subsection{Training Strategy} The overall optimization objectives consist of three trade-off terms: rate loss $\mathcal{L}_{\text{rate}}$, latent distortion loss $\mathcal{L}_{\text{ld}}$ and diffusion loss $\mathcal{L}_{\text{diff}}$. The loss function can be formulated as:
\begin{equation} 
\begin{aligned}
    \mathcal{L}=\lambda_{\text{rate}}\mathcal{L}_{\text{rate}} + \lambda_{\text{ld}}\mathcal{L}_{\text{ld}} + \lambda_{\text{diff}}\mathcal{L}_{\text{diff}},
\end{aligned}
\label{eq12}
\end{equation}
where $\lambda_{\text{rate}}$, $\lambda_{\text{ld}}$ and $\lambda_{\text{diff}}$ are the corresponding weights. However, we have found that the joint optimization described in \:\hyperref[eq12]{(12)} leads to instability of training and difficulty in convergence. In contrast, we propose a two-stage training strategy for the optimization of the latent compression module and conditional diffusion model respectively. 

In the first stage, we introduce the rate-distortion trade-off to optimize the LCM, which is described as:
\begin{align}
    \mathcal{L}_{\text{1st}}&=\mathcal{L}_{\text{rate}} + \lambda\mathcal{L}_{\text{ld}}, \nonumber\\
    \mathcal{L}_{\text{rate}}&=\mathbb{E}_{z_0\sim p_z}[-{\rm log_2}\mbox{\,}p_{\hat{y}}(\hat{y})]+\mathbb{E}_{z_0\sim p_z}[-{\rm log_2}\mbox{\,}p_{\hat{h}}(\hat{h})], \nonumber\\
    \mathcal{L}_{\text{ld}}&=\left\|\hat{z}-z_0 \right\|^2,
\label{eq13}
\end{align} 
where $\lambda$ is the Lagrange multiplier that controls the expected trade-off between rate and latent distortion.
$p_z$ is the distribution of latent representations obtained from input source images. 
$p_{\hat{y}}$ and $p_{\hat{h}}$ are the probability distribution of $\hat{y}$ and $\hat{h}$ for the entropy coding.

In the second stage, we finetune the decoding transform $\text{g}_\text{s}(\cdot)$ and $\text{h}_\text{s}(\cdot)$ of LCM to condition the denoising diffusion process adaptively. Since the SD model is pre-trained on natural images, we finetune the linear layers on our training set to improve the compression performance. The trainable parameters are illustrated in Fig.\:\hyperref[fig2]{2} and the loss function is formulated as follows:
\begin{equation} 
\begin{aligned}
    \mathcal{L}_{\text{2nd}}&=\mathbb{E}_{z_0,c,\epsilon,t}\left\|\epsilon- \epsilon_\theta(z_t,c,t)  \right\|^2 \\
    \text{with}\quad c &=(\hat{z},f_{\text{ms}}),
\end{aligned}
\end{equation}
where $c$ presents the conditional control that contains implicit and explicit guidance. 

==> sec/4_dataset.tex <==
\section{Datasets and image quality assessment metrics}\label{sec:Datasets and assessment metrics}
\subsection{Datasets}\label{sec:Datasets}
In this paper, we collect a new benchmark dataset named Cross-Modal Super-Resolution Dataset (CMSRD) to validate the proposed SGDM and hope to facilitate future research on large scale factor remote sensing image super-resolution. This dataset is composed of two parts: synthetic data and real-world data, with detailed information depicted in Table \ref{tab:cmsrd_dataset} and some examples of the image pairs shown in Fig. \ref{fig:dataset_examples}.

The CMSRD consists of triplets LR-Map-HR, all HR images are sourced from World Imagery, while all vector maps are obtained from Open Street Map. The synthetic dataset comprises 45,300 image pairs, with 45,000 pairs used for training and 300 pairs for testing. LR images are obtained by downsampling HR images by a factor of 32 using bicubic interpolation. The synthetic dataset is used to validate the effectiveness of introducing vector maps in large scale factor remote sensing image super-resolution. The real-world dataset consists of 50,754 image pairs, with 50,364 used for training and 390 for testing. In contrast to the synthetic dataset, LR images in the real-world dataset are sourced from the Sentinel-2 satellite series. We ensure 16$\times$ spatial size difference between HR and LR through bicubic resampling. As shown in Fig. \ref{fig:dataset_examples}, there exists content consistency and style gap among remote sensing images from different sources, which is one of the main issues to be explored in this work.

\subsection{Image quality assessment metrics}\label{sec:Assessment metrics}
To conduct a comprehensive evaluation of various remote sensing image super-resolution methods, we employ both full-reference and no-reference image quality assessment metrics. For assessing reconstruction fidelity, peak signal noise ratio (PSNR) and structure similarity (SSIM) \citep{wang2004image} calculated on the Y channel of the YCbCr color space are used. For the perceptual quality evaluation, full-reference metrics learned 
perceptual image patch similarity (LPIPS) \citep{zhang2018unreasonable} and deep image structure and texture similarity (DISTS) \citep{ding2020image} are employed. Furthermore, fréchet inception distance (FID) \citep{heusel2017gans} is used to gauge the distributional disparity between the ground truth images and the SR images. For no-reference image quality assessment, we use metrics such as multi-scale image quality transformer (MUSIQ) \citep{ke2021musiq} and CLIPIQA \citep{wang2023exploring}.

\begin{table*}
	\caption{Quantitative comparisons with different methods on the synthetic data for 32$\times$ SR and real-world data for 16$\times$ SR, where the bold font indicates the best performance. The symbols $\uparrow$ and $\downarrow$ respectively represent that higher or lower values indicate better performance.}
	\label{tab:quantitative comparison}
	\centering
	\begin{tabular}{ccccccccc}
		\hline
         Type &Metric &ESRGAN &SwinIR &LDM &ResShift &TTST &EDiffSR &SGDM/SGDM+\cr
        \hline
        \multirow{7}{*}{Synthetic} 
        &PSNR$\ \uparrow$ &20.26 &21.74 &20.12 &19.29 &\textbf{21.88} &20.32 &20.65\cr
        &SSIM$\ \uparrow$ &0.3233 &0.4029 &0.3121 &0.3021 &\textbf{0.4064} &0.2836 &0.3338\cr
        &LPIPS$\ \downarrow$ &0.4551 &0.8932 &0.4925 &0.4585 &0.8396 &0.4517 &\textbf{0.4344}\cr
        &DISTS$\ \downarrow$ &0.2561 &0.5528 &0.2609 &0.2537 &0.5001 &0.2480 &\textbf{0.2356}\cr
        &FID$\ \downarrow$ &70.67 &357.8 &42.43 &86.24 &295.3 &108.3 &\textbf{36.62}\cr
        &MUSIQ$\ \uparrow$ &38.13 &19.99 &39.40 &37.31 &17.77 &38.54 &\textbf{40.30}\cr
        &CLIPIQA$\ \uparrow$ &0.5951 &0.2683 &0.6116 &0.4546 &0.2471 &0.4590 &\textbf{0.6238}\cr \hline
        
        \multirow{5}{*}{Real world}
        &LPIPS$\ \downarrow$ &\textbf{0.5592} &0.9137 &0.6006 &0.6218 &0.9108 &0.6064 &0.5978\cr
        &DISTS$\ \downarrow$ &\textbf{0.3124} &0.5948 &0.3225 &0.3516 &0.5615 &0.3458 &0.3231\cr
        &FID$\ \downarrow$ &98.15 &423.2 &49.40 &166.4 &359.7 &156.1 &\textbf{44.81}\cr
        &MUSIQ$\ \uparrow$ &44.23 &20.51 &46.70 &44.41 &19.11 &42.21 &\textbf{48.92}\cr
        &CLIPIQA$\ \uparrow$ &0.4727 &0.2581 &0.5956 &0.3989 &0.2547 &0.4385 &\textbf{0.6064}\cr \hline
	\end{tabular}
\end{table*}

==> sec/5_exp.tex <==
\section{Experiments}\label{sec:Experiments}
\subsection{Implementation details}\label{sec:Implementation details}
Our SGDM is built based upon the Stable Diffusion 2.1-base model. We implement the proposed SGDM using the PyTorch framework and all experiments are conducted on two NVIDIA GeForce RTX 3090 GPUs. 

The training phase consists of two stages. Firstly, we fine-tune the Stable Diffusion model using the loss function in Equation \ref{equ:r3_l2_loss}. During this phase, we optimize the parameters of content-style encoder, adapter, and the linear layers of U-net, which amounts to a total of 148M trainable parameters. We train the model with a batch size of 32 for 150K steps, and employ the AdamW optimizer with a learning rate of $5 \times 10^{-5}$. Subsequently, we utilize the trained style encoder to re-calculate style vectors ($\mu$ and $\sigma$) for all HR images in the training set and use them to train the SFlow model. The SFlow architecture follows the structure proposed in \cite{dinh2016density}, with hidden layer dimensions set to 16, 32, 32, 64 and the number of affine coupling layers set to 8. We employ two separate SFlow models for the distributions of $\mu$ and $\sigma$. We use the Adam optimizer with a learning rate of $4 \times 10^{-4}$, and the training of SFlow can be completed within two hours.

It is important to note that our style correction module (SCM), designed as a plug-and-play module, is not required when experimenting on synthetic datasets (referred to as SGDM). However, for real-world datasets, we integrate the SCM to address the style discrepancies between LR and HR images (referred to as SGDM+). Considering that previous methods for large scale factor super-resolution are only suitable for specific types of scenes, such as face \citep{chan2021glean, gu2020image, menon2020pulse}, here, we select some state-of-the-art (SOTA) SR methods for natural images to do the comparison, such as ESRGAN \citep{wang2018esrgan}, SwinIR \citep{liang2021swinir} and ResShift\citep{yue2024resshift}. LDM \citep{rombach2022high} is also chosen as a comparison method to validate the effectiveness of the semantic and style guidance we proposed. In addition, we also select two SOTA methods for remote sensing image super-resolution for comparison, \ie, the EDiffSR \citep{xiao2023ediffsr} and TTST \citep{xiao2024ttst}. For the sake of fairness, all methods are trained on our CMSRD dataset using the source code and hyper-parameter settings provided by those papers. It should be noted that the original hyper-parameter settings of ESRGAN results in convergence issues in scenarios of large scale factor super-resolution. Therefore, we adjust the scale of its loss functions to make it better suited for this task.

\subsection{Experiments on synthetic data}\label{sec:Experiments on synthetic data}
\subsubsection{Quantitative SR results}\label{sec:Quantitative results(syc)}

Table \ref{tab:quantitative comparison} presents 32$\times$ SR results of different methods compared on synthetic data. Transformer-based regression models, such as SwinIR and TTST, exhibit the highest PSNR and SSIM scores. However, these methods often produce over smooth SR images, which negatively impacts perceptual quality, as reflected by the low LPIPS, DISTS, FID, MUSIQ, and CLIPIQA scores. Meanwhile, ESRGAN, ResShift, and EDiffSR, as generative models based on GAN, diffusion, and SDE, exhibit similar performance. They show improved perceptual quality but still struggle for maintaining fidelity, leading to lower PSNR and SSIM. However, our proposed SGDM outperforms in both aspects and achieves the best balance between perceptual quality and fidelity. In addition to achieving the best performance across all perceptual metrics, SGDM also achieves relatively high PSNR and SSIM scores. On one hand, SGDM can utilize coarse texture and structural information from LR images and explicit semantic information from vector maps to effectively improve the fidelity of the reconstruction results; on the other hand, by leveraging the powerful generative prior of the Stable Diffusion, SGDM is still able to recover detailed textures that match real scenes even in extreme large factor super-resolution scenarios. Notably, despite relatively good perceptual metrics of LDM, it has a significantly higher number of trainable parameters (865M) compared to SGDM (148M), which highlights the efficiency and effectiveness of our network architecture.

\subsubsection{Qualitative SR results}\label{sec:Qualitative results(syc)}
In Fig. \ref{fig:sync_qualitative}, we present a visual comparison of super-resolution results using different methods on the synthetic dataset. Due to the low spatial resolution of the LR input, a substantial amount of high-frequency information is lost and there exhibit significant semantic ambiguity. Consequently, traditional transformer-based regression models (SwinIR and TTST) can only produce overly smooth results, struggling to recover the lost high-frequency texture details. Among generative methods, ESRGAN and ResShift perform relatively better. ESRGAN can recover most of the high-frequency details, but suffer from serious distortion and deformation of the reconstructed ground objects. In contrast to ESRGAN, ResShift can reconstruct more regular shapes of objects, but it cannot recover as much high-frequency details as ESRGAN. LDM can generate richer and more realistic details compared to ESRGAN and ResShift. However, due to the lack of semantic guidance, positions and shapes of the generated objects exhibit some disarray. Thanks to the precise semantic guidance provided by vector maps and the powerful generative capabilities of Stable Diffusion, the proposed SGDM effectively addresses the problem of semantic ambiguity and the loss of high-frequency details, thereby achieving reconstruction results that balance realism and fidelity.

\begin{figure*}[htp]
    \centering
    \includegraphics[width=\linewidth]{figures/r5/sync_qualitative.png}
    \caption{Visual comparison of 32$\times$ super-resolution on synthetic dataset. We select four representative scenes: residential areas, roads, squares, and factories.}
    \label{fig:sync_qualitative}
\end{figure*}

\begin{figure*}[htp]
    \centering
    \includegraphics[width=\textwidth]{figures/r5/real_qualitative.png}
    \caption{Visual comparison of 16$\times$ super-resolution on real-world dataset.}
    \label{fig:real_qualitative}
\end{figure*}

\subsection{Experiments on real-world data}\label{sec:Experiments on real-world data}
\subsubsection{Quantitative SR results}\label{sec:Quantitative results(real)}
Table \ref{tab:quantitative comparison} shows the evaluation results of different comparative methods on real-world data for 16$\times$ SR. Our proposed SGDM+ achieves the best performance on all no-reference metrics. However, it lags slightly behind ESRGAN in two full-reference perceptual metrics. This is because during testing, we do not provide any style guidance images and instead get completely random style vectors by sampling from the latent space of SFlow. Therefore, one-to-one evaluation metrics cannot fully demonstrate the advantages of SGDM+. However, the lower FID indicates that SGDM+ can better capture the distribution of HR images compared to other methods. This is because SGDM+ can independently model the style of HR through the SCM module, effectively overcoming the style misalignment between LR and HR in real-world scenarios.

\begin{figure*}[htp]
    \centering
    \includegraphics[width=\textwidth]{figures/r5/style-guidance.png}
    \caption{Visual comparison between reconstruction results given different style guidance images.}
    \label{fig:style_guidance}
\end{figure*}

\begin{figure*}[htp]
    \centering
    \includegraphics[width=\textwidth]{figures/r5/style-sample.png}
    \caption{Visual comparison between reconstruction results with different sampling seeds for normalizing flow.}
    \label{fig:style_sample}
\end{figure*}

\subsubsection{Qualitative SR results}\label{sec:Qualitative results(real)}
Visual comparisons between different methods on real-world data are shown in Fig. \ref{fig:real_qualitative}. Due to the entanglement between content attributes and style attributes, the results provided by all comparative methods tend to have the average style of HR images, for example SR images tend to be darker. SGDM+ can perform style sampling based on the normalizing flow model, forming a more flexible solution space. Additionally, we find that due to the style differences between LR and HR in real-world datasets, some comparative methods even have difficulty converging during training (such as ResShift and EDiffSR), resulting in severely distorted SR results. ESRGAN, while capable of producing relatively accurate ground objects, falls short in generating rich textures. While LDM can generate results with higher realism, it often generates ground objects that do not match the ground truth due to the lack of accurate semantic guidance. SGDM+, on the other hand, obtains SR results that combine fidelity and realism under the guidance of vector maps and the support of pre-trained Stable Diffusion model.

\subsubsection{SR results of different style control strategies}\label{sec:Style control}
\textbf{Style guidance from example HR image.}
In many instances, addressing remote sensing image super-resolution often involves leveraging heterogeneous or historical remote sensing images as references. For example, \cite{dong2021rrsgan} proposed using HR remote sensing images captured by other satellite platforms as references to assist in the super-resolution process, thereby obtaining more realistic texture details. In contrast to their content-based reference methods, we advocate using HR remote sensing images as a style reference to overcome the style misalignment between LR and HR images. During inference, our framework can reuse the trained style encoder to extract the style vectors of the style guidance images, and then apply style injection on the LR feature maps through the AdaIN module. As shown in Fig. \ref{fig:style_guidance}, when providing different style guidance images, the model can perform instance-level style guidance (such as colors of buildings and roads, and the density of vegetation), thereby obtaining more controllable reconstruction results.

\textbf{Style sampled from fitted probabilistic distribution.}
In the most challenging scenario where no style guidance images are available, we can directly sample from the SFlow to acquire style vectors for super-resolution. It should be noted that due to the limited training data, the normalizing flow model can only approximate (rather than fully simulate) the style distribution of HR images. Therefore, compared to style guidance, style sampling will lower the quality and increase the uncertainty of the reconstruction results. As shown in Fig. \ref{fig:style_sample}, by changing the random seed for sampling from the style normalizing flow, we can obtain reconstruction results that are consistent in content but diverse in style. Due to the lack of appropriate style guidance, these results represent the lower bound of the performance of SGDM+ under extreme conditions (which is also the performance of SGDM+ recorded in Table \ref{tab:quantitative comparison}).

\begin{table*}
	\caption{Ablation study of our method (SGDM) on the synthetic split of CMSRD.}
	\label{tab:ablation_study}
	\centering
	\begin{tabular}{cccccc}
		\hline
         \makecell[c]{LR condition} &\makecell[c]{Vector map prior} &\makecell[c]{Stable Diffusion prior} &\makecell[c]{SPADE block} &LPIPS$\ \downarrow$ &FID$\ \downarrow$\cr
        \hline
        $\checkmark$ &$\checkmark$ &$\times$ &$\checkmark$ &0.8498 &277.2 \cr
        $\checkmark$ &$\times$ &$\checkmark$ &$\times$ &0.4652 &42.43 \cr
        $\checkmark$ &$\checkmark$ &$\checkmark$ &$\times$ &0.4478 &43.83 \cr
        $\checkmark$ &$\checkmark$ &$\checkmark$ &$\checkmark$ &\textbf{0.4344} &\textbf{36.63} \cr\hline
	\end{tabular}
\end{table*}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\columnwidth]{figures/r6/effectiveness-sg.png}
    \caption{Performance of different methods on the synthetic dataset. `SGDM-shuffle-map' represents using vector maps completely unrelated to ground truth.}
    \label{fig:effectiveness-sg}
\end{figure}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\columnwidth]{figures/r6/sg-visual.png}
    \caption{Visualization of the reconstruction results of SGDM given  vector map as semantic guidance. The reconstruction results of the first two rows are less affected by vector maps, while the last two rows are more significantly influenced.}
    \label{fig:sg-visual}
\end{figure}


==> sec/6_ablation.tex <==
\section{Ablation studies}\label{sec:Ablation studies}
\subsection{Effectiveness of diffusion prior}\label{sec:Effectiveness of diffusion prior}
The powerful generative capabilities of pre-trained Stable Diffusion can significantly enhance the visual quality of reconstruction outcomes. To assess its efficacy, we conduct an experiment where we employ our proposed content guided module (CGM) alone, bypassing the pre-trained Stable Diffusion as a prior. As demonstrated in the first row of Table \ref{tab:ablation_study}, the absence of the pre-trained Stable Diffusion prior leads to significantly lower perceptual quality in the reconstruction, due to the inherent limitations of traditional regression models in bridging the substantial spatial resolution disparity between LR and HR images.

\subsection{Effectiveness of semantic guidance}\label{sec:Effectiveness of semantic guidance}
For our proposed SGDM, vector maps serve as semantic guidance to enhance the fidelity of the reconstruction results. We evaluate the effectiveness of vector maps from two perspectives: whether vector maps are useful for improving the results, and whether the method we introduce vector maps is the most effective. For the former, we use only LR as the condition to guide the generation process of the diffusion model. For the latter, we eliminate all SPADE modules in the content guided module and simply merge the features of LR and the vector map by concatenation. The results of these experiments are presented in the second and third rows of Table \ref{tab:ablation_study}. These experiments demonstrate that incorporating vector maps through concatenation can also improve reconstruction fidelity. The SPADE module, as a spatially adaptive feature modulation technique, exploits the full potential of the semantic information from vector maps, thus yielding better results compared to simple concatenation.

Additionally, we also conduct some experiments to test the robustness of SGDM. By inputting vector maps that are entirely unrelated to the ground truth, we can assess the reliance of the model on vector maps. As depicted in Fig. \ref{fig:effectiveness-sg}, even with irrelevant vector maps, SGDM still generates relatively plausible reconstructions, outperforming LDM and ESRGAN. Conversely, when vector maps lack accurate semantic guidance, performance of the SGDM decreases, indicating the efficacy of vector map integration. From Fig. \ref{fig:sg-visual}, it can be observed that the reconstruction results of some remote sensing images, such as large scale buildings and cluttered texture areas, are not affected by the inaccurate semantic guidance from the vector maps. However, for dense urban scenes, the model heavily relies on semantic information provided by vector map, thereby leading to less satisfactory results.

\begin{figure}[tp]
    \centering
    \includegraphics[width=\columnwidth]{figures/r6/effectiveness-scm.png}
    \caption{Performance of SGDM+ under different style guidance strategies. `Sample style' refers to style sampling through normalization flows. `Shuffle style' denotes style guidance using randomly chosen HR images. `GT style' indicates directly using the ground truth for style guidance.}
    \label{fig:effectiveness-scm}
\end{figure}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\columnwidth]{figures/r6/style_compare.png}
    \caption{The t-SNE visualization of style vectors. It can be observed that there is a clear distribution difference between LR and HR, while our style normalization flow fits well into the style distribution of HR.}
    \label{fig:style_compare}
\end{figure}

\subsection{Effectiveness of style modelling}\label{sec:Effectiveness of style transfer}
To tackle the issue of style inconsistency between LR and HR images in real-world scenarios, we've developed a style correction module to enhance the capability of the model for style modelling. During testing, we can either employ the style encoder for style guidance or utilize normalization flow for random style sampling. Therefore, theoretically, completely random style sampling and using the ground truth for style guidance respectively represent the lower and upper bounds of the performance of SGDM+. Additionally, we can input randomly selected HR images for style guidance, which represents the average performance of SGDM+ under general conditions. We conduct these three inference methods separately and compare the results with the approach of not using the style correction module (\ie, SGDM). The obtained results are shown in Fig. \ref{fig:effectiveness-scm}. It can be observed that using the ground truth as style guidance and random style sampling achieve the best and worst reconstruction results. Notably, using randomly selected HR images for style guidance also produces favorable results, surpassing the model without the style correction module. These findings robustly attest to the efficacy and substantial practical applications of our proposed style correction module.

To visually inspect the distinct style distributions between LR and HR, we present a visualization of style vectors for 10,000 randomly chosen training pairs in Fig. \ref{fig:style_compare}. The comparison clearly illustrates a substantial difference in style distribution between HR and LR (denoted as `HR style space' and `LR style space' in Fig. \ref{fig:motivation}). Our proposed style normalization flow effectively aligns with the HR image style distribution. During testing, by directly sampling from the normalization flow, we can provide useful style priors to the model, thereby enhancing the reconstruction fidelity.

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth]{figures/r6/task_segment.png}
    \caption{Visual comparison of semantic segmentation results from different super-resolution methods.}
    \label{fig:task_segment}
\end{figure*}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\columnwidth]{figures/r6/task_metric.png}
    \caption{Quantitative comparison of scene recognition and semantic segmentation results among different super-resolution methods.}
    \label{fig:task_metric}
\end{figure}


\subsection{Evaluate usability of SR images on downstream vision tasks}\label{sec:downstream_tasks}
The evaluation of natural image quality primarily relies on quantitative metrics and visual appeal. However, the value of remote sensing images lies in their performance on relevant analysis tasks. To assess the reconstruction quality of various SR methods comprehensively, we choose two representative downstream tasks (scene recognition and semantic segmentation) to showcase the superiority of our proposed method in perceptual quality. Due to the absence of the ground truth, we leverage a pre-trained remote sensing foundation model (RVSA \citep{wang2022advancing}) with strong generalization capabilities to analyze the SR results. Our focus is on the relative performance of SR results compared to HR images in the context of these tasks, not the absolute accuracy of SR results. Thus all metrics, such as classification accuracy and mean intersection over union (mIoU), are computed using HR analysis results as a reference.

\textbf{Scene recognition.}
The scene recognition task aims to classify input remote sensing images, enabling a comprehensive assessment of global semantic consistency between SR results and HR. We employ the RVSA model fine-tuned on the UC Merced Land-Use dataset \citep{yang2010bag} to classify the test set images in the real-world CMSRD dataset. As shown in Fig. \ref{fig:task_metric}, our proposed SGDM+ achieves the highest classification accuracy (\ie, the most similar classification results compared to HR), with a top-5 accuracy close to 80\%. This indicates that the SR results of SGDM+ have the highest fidelity for machine perception. Notably, all generative models, including SGDM+, outperform regression models like TTST and SwinIR, highlighting the limitations of pixel-level loss for machine vision tasks.

\textbf{Semantic segmentation.}
The semantic segmentation task aims to classify each pixel of a given remote sensing image. We utilize this task to evaluate the consistency between SR results and HR in terms of local semantics. We use the RVSA model fine-tuned on the LoveDA dataset \citep{wang2021loveda} to segment the test images, and the mean intersection over union (mIoU) of segmentation results is displayed in Fig. \ref{fig:task_metric}. Consistent with scene recognition, SGDM+ delivers the best segmentation outcomes, significantly outperforming other methods. In Fig. \ref{fig:task_segment}, visual comparisons reveal that most comparative methods struggle with precise ground object reconstruction, while SGDM+ provides the closest results to HR, particularly for buildings and roads, underscoring the promising prospects of our proposed method.


==> sec/7_conclusion.tex <==
\section{Conclusion}\label{sec:Conclusion}
In this paper, we propose a novel framework (SGDM) for large scale factor remote sensing image super-resolution. To address challenges such as semantic inaccuracies and texture blurriness commonly encountered in this task, we utilize vector maps to provide semantic guidance and exploit the powerful generative capabilities of the pre-trained Stable Diffusion model to generate more realistic SR images. Additionally, considering the style differences between LR and HR caused by the sensor-specific imaging characteristics in real-world scenarios, we develop a method for extracting style information and modeling its probability distribution. During testing, diverse outputs can be obtained through style guidance or style sampling.

Extensive experiments are conducted on our proposed CMSRD dataset. Both qualitative and quantitative experiments demonstrate the superiority of our proposed framework. Comprehensive ablation experiments validate the necessity of key components in SGDM, including vector maps, generative priors, and style correction module. Finally, we further demonstrate the application prospects of our proposed framework through two downstream tasks: scene recognition and semantic segmentation. In future work, we will further explore the feasibility of large scale factor remote sensing image super-resolution by introducing richer explicit priors (such as digital elevation maps, historical remote sensing images, etc.) and higher-quality generative priors (such as pre-trained models for remote sensing images).

